Control Synthesis Along Uncertain Trajectories Using Integral Quadratic Constraints

The paper presents a novel approach to synthesize robust controllers for nonlinear systems along perturbed trajectories. The approach linearizes the system with respect to a reference trajectory. In contrast to existing methods rooted in robust linear time-varying synthesis, the approach accurately includes perturbations that drive the system away from the reference trajectory. Hence, the controller obtained in the linear framework provides a significantly more robust nonlinear performance. The calculation of the controller is derived from robust synthesis approaches rooted in the integral quadratic constraints framework. The feasibility of the approach is demonstrated on a pitch tracker design for a space launcher.

==> figures/IQCAnalysisStep.tex <==
% Define Colors
\definecolor{mycolor1}{HTML}{367D7D}
\definecolor{mycolor2}{HTML}{D33502}
\definecolor{mycolor3}{HTML}{FAA818}
\definecolor{mycolor4}{HTML}{41A30D}
\definecolor{mycolor5}{HTML}{FFCE38}
\definecolor{mycolor6}{HTML}{6EBCBC}
\definecolor{mycolor7}{HTML}{37526D}

\colorlet{plant}{mycolor5!40!white}
\colorlet{unc}{mycolor6!40!white}
\colorlet{closedloop}{gray!20!white}
\colorlet{controller}{mycolor4!30!white}
\colorlet{dist}{mycolor3!60!white}
\colorlet{marker}{mycolor7}
\colorlet{algo}{mycolor3!60!white}
\colorlet{miscplot}{mycolor2}
\colorlet{clplot}{mycolor2}

% Arrow Style
\tikzset{>=stealth'}

\begin{tikzpicture}[thick,rounded corners = 0.5mm]
\begin{scope}[shift={(-0.9,0)}]
\draw[densely dotted,fill=closedloop,fill opacity=1] (0.1,-2.1) rectangle (3,0.8);
\end{scope}
\draw [fill=plant] (0,-0.7) rectangle node{$G$}(1.3,0.6);
\draw [->](0,0.1) -- (-1.2,0.1);
\draw [->](0,-0.2) -- (-1.2,-0.2);
\draw [->](0,0.4) -- (-1.2,0.4);
\draw [->](2.4,0) -- (1.3,0);
\draw [->](2.4,0.4) -- (1.3,0.4);
\node at (2.6,0) {$d$};
\node at (0.7,-2.4) {\footnotesize$N:=\mathcal{F}_l(G,K)$};
\node at (2.6,0.4) {$w$};
\node at (-1.5,0.4) {$v$};
\node at (-1.5,0.1) {$e_I$};
\node at (-1.5,-0.2) {$e_E$};
\draw [fill=controller] (0.3,-1.2) rectangle node{$K$}(1.1,-1.9);
\draw [->](0,-0.5) -- (-0.4,-0.5) -- (-0.4,-1.5) -- (0.3,-1.5);
\draw [->](1.1,-1.5) -- (1.7,-1.5) -- (1.7,-0.5) -- (1.3,-0.5);
\node at (1.9,-1.2) {$u$};
\node at (-0.6,-1.2) {$y$};
\end{tikzpicture}

==> figures/LFTNominalSynthesis.tex <==
% Define Colors
\definecolor{mycolor1}{HTML}{367D7D}
\definecolor{mycolor2}{HTML}{D33502}
\definecolor{mycolor3}{HTML}{FAA818}
\definecolor{mycolor4}{HTML}{41A30D}
\definecolor{mycolor5}{HTML}{FFCE38}
\definecolor{mycolor6}{HTML}{6EBCBC}
\definecolor{mycolor7}{HTML}{37526D}

\colorlet{plant}{mycolor5!40!white}
\colorlet{unc}{mycolor6!40!white}
\colorlet{closedloop}{gray!20!white}
\colorlet{controller}{mycolor4!30!white}
\colorlet{dist}{mycolor3!60!white}
\colorlet{marker}{mycolor7}
\colorlet{algo}{mycolor3!60!white}
\colorlet{miscplot}{mycolor2}
\colorlet{clplot}{mycolor2}

% Arrow Style
\tikzset{>=stealth'}

\begin{tikzpicture}[thick,scale=0.9,rounded corners = 0.5mm]
\draw [->](0,0.9) -- (-1.1,0.9);
\draw [->](0,0.5) -- (-1.1,0.5);
\draw [->](2.2,0.7) -- (1.2,0.7);
\node at (2.4,0.7) {$d$};
\node at (-1.4,0.9) {$e_I$};
\node at (-1.4,0.5) {$e_{E}$};
\draw [fill=controller]  (0.2,-0.5) rectangle node{$K$}(1,-1.2);
\draw [->](0,0.2) -- (-0.5,0.2) -- (-0.5,-0.8) -- (0.2,-0.8);
\draw [->](1,-0.8) -- (1.7,-0.8) -- (1.7,0.2) -- (1.2,0.2);
\node at (-0.7,-0.3) {$y$};
\node at (1.9,-0.3) {$u$};
\draw [fill=blue,fill opacity=0.1] (0,-0.1) rectangle node{$G$}(1.2,1.2);
\draw (0,-0.1) rectangle node{$G$}(1.2,1.2);
\end{tikzpicture}

==> figures/Log_LSHAD_new_Pseudocode_updt_alt.tex <==
\begin{algorithm}[ht!]
\caption{Uncertain Trajectory Synthesis}
\label{Alg:Log-L-SHADE}
\begin{algorithmic}[1]

\State {\textbf{Input:} $n_\text{P,max}$, $n_\text{P,min}$, $i_\text{max}$, $k_{CR}$,  $k_{F}$, $H$, $\mathcal{M}$, $s_\text{min}$, $s_\text{max}$, $\gamma_\text{lim}$, $M_\text{Log}^{(0)}$, $k_\text{IQC}$, $\gamma_\text{LB}$, $\gamma_\text{UB}$, $\epsilon_\text{BS}$}
\State{\textbf{Output:} $\gamma_\text{best}$, $M_\text{Log,best}$}
\State{\textbf{Initialize:} $S_F$, $S_{CR}$}
\State{Scale original IQC norm bound by $k_\text{IQC}$}
\While{Less than $20\%$ valid initial members}
\State{Generate random initial population $\{M_{\text{log},j}^{(1)}\}_{j=1}^{n_\text{P}}$}
\State{Calculate $\gamma(M_{\text{Log},j}^{(i)})$ via bisection}
\EndWhile
\State{Find current best solution $M_\text{Log,best}$ and fitness $\gamma_\text{best}$}
\State{Set IQC norm bound upscaling threshold $n_\text{P,IQC}=n_\text{P,max}$}
	
\While{($i \le i_\text{max}$ OR $\gamma_\text{best}>\gamma_\text{lim}$) AND $k_\text{IQC}<1$}
	\State{$i = i+1$}
	\If{($\gamma_\text{best} \le \gamma_\text{lim}$ OR $n_{P}<0.8 n_\text{P,IQC}$) AND \newline
	\hspace*{1.54em}$k_\text{IQC}<1$}
	\State{Set $n_\text{P,IQC} = n_\text{P}$ and $k_\text{IQC}  = \text{min}(3k_\text{IQC}, 1)$}
	\State{Upscale norm bound, recalculate $\gamma(M_{\text{Log},j}^{(i-1)})$ with\newline
	\hspace*{3.1em}user $\gamma_\text{UB}$, and update $M_\text{Log,best}$ and $\gamma_\text{best}$}
	\EndIf
	\For{$j =1$ to $n_\text{P}$}
		\State{Calculate $M_{\text{Log},j}^{(i)}$ using (\ref{eq:MutationOp}) and crossover, \newline
		\hspace*{3.0em}enforce boundaries, and  ${M}^{(i)}_{\text{Log},j} \in \mathcal{M}$}
		\If{RDE is solvable for ${M}^{(i)}_{\text{Log},j}$ and $\gamma({M}^{(i-1)}_{\text{Log},j})$}
		\State{Execute bisection with $\gamma_\text{UB} = \gamma(M^{(i-1)}_{\text{Log},j})$}
		\Else
			\State{Skip bisection and set $\gamma(M_\text{Log,j}^{(i)}) = 10^{20}$}
		\EndIf
	\If{$\gamma(M_{\text{Log},j}^{(i)})>\gamma(M_{\text{Log},j}^{(i-1)})$}
		{$M_{\text{Log},j}^{(i)}=M_{\text{Log},j}^{(i-1)}$} 
	\EndIf
	\EndFor
	\State{Update $S_F$ and $S_{CR}$ based on successful $F$ and $CR$}
	\State{Identify current best solution $M_\text{Log,best}$ and fitness $\gamma_\text{best}$}
	\State{Update population $n_\text{P}$ size via (\ref{eq:PopSizeUp}) and remove worst \newline
	\hspace*{1.54em}solutions from $\{M_{\text{Log},j}^{(i)}\}_{j=1}^{n_\text{P}}$}
\EndWhile


\end{algorithmic}

\end{algorithm}



==> figures/ScaledPlant.tex <==
% Define Colors
\definecolor{mycolor1}{HTML}{367D7D}
\definecolor{mycolor2}{HTML}{D33502}
\definecolor{mycolor3}{HTML}{FAA818}
\definecolor{mycolor4}{HTML}{41A30D}
\definecolor{mycolor5}{HTML}{FFCE38}
\definecolor{mycolor6}{HTML}{6EBCBC}
\definecolor{mycolor7}{HTML}{37526D}

\colorlet{plant}{mycolor5!40!white}
\colorlet{unc}{mycolor6!40!white}
\colorlet{closedloop}{gray!20!white}
\colorlet{controller}{mycolor4!30!white}
\colorlet{dist}{mycolor3!60!white}
\colorlet{marker}{mycolor7}
\colorlet{algo}{mycolor3!60!white}
\colorlet{miscplot}{mycolor2}
\colorlet{clplot}{mycolor2}

% Arrow Style
\tikzset{>=stealth'}

\begin{tikzpicture}[thick,rounded corners = 0.5mm]
\draw [fill=closedloop] (0,-0.3) rectangle node{$N$}(1.4,1.2);
\draw [fill=dist] (2,-0.3) rectangle node{$\frac{1}{\gamma}$}(2.5,0.4);
\draw [fill=unc] (1.9,0.6) rectangle node{$M_{w}^{-\frac{1}{2}}$}(2.8,1.2);
\draw [fill=unc] (-1.1,0.6) rectangle node{$M_{v}^{\frac{1}{2}}$}(-0.39,1.2);
\draw [->](0,0.4) -- (-1.5,0.4);
\draw [->](0,0) -- (-1.5,0);
\draw [->](0,0.9) -- (-0.4,0.9);
\draw [->](2,0.1) -- (1.4,0.1);
\draw [->](1.9,0.9) -- (1.4,0.9);
\draw [->](3.09,0.9) -- (2.8,0.9);
\draw [->](3.1,0.1) -- (2.5,0.1);
\draw [->](-1.1,0.9) -- (-1.5,0.9);
\node at (1.7,0.4) {$d$};
\node at (3.3,0.1) {$\tilde{d}$};
\node at (1.7,1.2) {$w$};
\node at (3.29,0.9) {$\tilde{w}$};
\node at (-0.2,1.2) {$v$};
\node at (-1.8,0.9) {$\tilde{v}$};
\node at (-1.8,0.4) {$e_I$};
\node at (-1.8,0) {$e_E$};
\end{tikzpicture}

==> figures/ScaledPlantSynthesisStep.tex <==
% Define Colors
\definecolor{mycolor1}{HTML}{367D7D}
\definecolor{mycolor2}{HTML}{D33502}
\definecolor{mycolor3}{HTML}{FAA818}
\definecolor{mycolor4}{HTML}{41A30D}
\definecolor{mycolor5}{HTML}{FFCE38}
\definecolor{mycolor6}{HTML}{6EBCBC}
\definecolor{mycolor7}{HTML}{37526D}

\colorlet{plant}{mycolor5!40!white}
\colorlet{unc}{mycolor6!40!white}
\colorlet{closedloop}{gray!20!white}
\colorlet{controller}{mycolor4!30!white}
\colorlet{dist}{mycolor3!60!white}
\colorlet{marker}{mycolor7}
\colorlet{algo}{mycolor3!60!white}
\colorlet{miscplot}{mycolor2}
\colorlet{clplot}{mycolor2}

% Arrow Style
\tikzset{>=stealth'}

\begin{tikzpicture}[thick,scale=1,rounded corners = 0.5mm,every node/.style={scale=1}]
\draw [fill=unc] (0,0) rectangle node{$G_{scl}$}(1.2,1.2);
\draw [->](0,0.4) -- (-1.1,0.4);
\draw [->](0,0.7) -- (-1.1,0.7);
\draw [->](0,1) -- (-1.1,1);
\draw [->](2.2,0.6) -- (1.2,0.6);
\draw [->](2.2,1) -- (1.2,1);
\node at (2.4,0.6) {$\tilde{d}$};
\node at (2.4,1) {$\tilde{w}$};
\node at (-1.4,0.4) {$e_E$};
\node at (-1.4,0.7) {$e_I$};
\node at (-1.3,1) {$\tilde{v}$};
\draw [fill=controller] (0.2,-0.5) rectangle node{$K$}(1,-1.2);
\draw [->](0,0.2) -- (-0.6,0.2) -- (-0.6,-0.8) -- (0.2,-0.8);
\draw [->](1,-0.8) -- (1.8,-0.8) -- (1.8,0.2) -- (1.2,0.2);
\node at (-0.8,-0.3) {$y$};
\node at (2,-0.3) {$u$};
\end{tikzpicture}
